Origins of carbon-enhanced metal-poor stars

We investigate the nature of carbon-enhanced metal poor (CEMP) stars in Milky Way (MW) analogues selected from the EAGLE cosmological hydrodynamical simulation. The stellar evolution model in EAGLE includes the physics of enrichment by asymptotic giant branch (AGB) stars, winds from massive stars, and type I and type II supernovae (SNe). In the simulation, star formation in young MW progenitors is bursty due to efficient stellar feedback, which causes poor metal mixing leading to the formation of CEMP stars with extreme abundance patterns. In this scenario, two classes of CEMP stars emerge: those mostly enriched by low-metallicity type II SNe with low Fe yields that drive galactic outflows, and those mostly enriched by AGB stars when a gas-poor progenitor accretes pristine gas. The first class resembles CEMP-no stars with high [C/Fe] and low [C/O], the second class resembles CEMP-s stars overabundant in s-process elements and high values of [C/O]. This scenario explains several trends seen in data: (i) the increase in the scatter and median of [C/O] at low and decreasing [O/H], (ii) the trend of stars with very low [Fe/H] or [C/H] to be of type CEMP-no, and (iii) the reduction in the scatter of [{\alpha}/Fe] with atomic number in metal poor stars. In this interpretation CEMP-no stars were enriched by the stars that enabled galaxies to reionise the Universe.

==> AGB.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{AGB origin for the [C/O] upturn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Equipped with the abundance of elements for the stars in the {\sc eagle} simulation we can track carbon in the stars that end up in the Milky Way today. According to standard enrichment models a trend of increasing [C/O] with increasing [O/H] is generally expected that simply is a reflection of the gradual increase in metallicity with the age of the Universe. The lowest metallicity metal poor stars that are typically found in the halo of the Milky Way should be having lower amount of carbon and the newly born disc stars having near solar abundance ratios.


However observations reveal a surprising upturn in [C/O] ratios at low metallicities  \citep{Akerman04,Fabbian09,Pettini14}. Moreover it is speculated that the upturn is a manifestation of the enrichment by  PopIII stars, and the population synthesis models that include the yields from PopIII can produce higher [C/O] at low metallicities (cyan curve in panel c, Fig.~\ref{fig_CO}).

Interestingly we also recover the upturn for the stars in the Milky Way type galaxies in the {\sc eagle} simulation (red curve in Panel a Fig.~\ref{fig_CO}) which is surprising  since in our simulations we do not use the yields from PopIII. Instead it actually is a consequence of the metal enrichment in pristine gas by the AGB population.% (Fig.~\ref{fig_CO}).

The question then arises whether the AGB stars in the early galaxies were aged sufficiently by the redshift 6 so as to produce significant amounts of carbon. The general perception would be that the enrichment due to AGB need roughly a gigayear, however, we note that the yield from AGB increases monotonically and significant even at 100 Myr (solid curve in panel d, Fig.~\ref{fig_CO}). The mean age of stellar population at $z=6$ is approximately half a gigayear, and therefore, the first generation of AGBs should be able to supply adequate amount of carbon at $z\geq 6$.% and to leave imprints in the old stars around us in the present day Universe.

Not only the abundance of carbon is higher but the abundance of oxygen is also lower since the upturn is seen in the ratio [C/O] and at low [O/H]. It is important since apart from the AGB, the SNII are also a viable enrichment agent and they can produce both carbon and oxygen. In fact the mean solar abundance ratio of carbon and oxygen that we see today is due to a combined contribution from SNe and AGB. However the trend of higher [C/O] at low [O/H] signals a lack of oxygen. Since the oxygen comes primarily from SNII with AGB contributing only in trace amounts therefore the upturn in [C/O] is a consequence of pure AGB enrichment. This is also evident in Panel d, in which the star particles with higher [C/O] acquire most of there metal mass from AGB (red particles in Fig.~\ref{fig_CO}).

% The question then arises that The fact that this channel was also operating apart from the AGB the oxygen abundances would have increased since the type they produce significant amount of oxygen. however the upturn at lower [O/H] implies a decreasing oxygen with increasing carbon, which is possible if the enrichment occurred only via the AGB channel.


==> Mixing.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% 
\section{Poor mixing and its consequences for metal poor stars}
%%%%%%%%%%%%%%%%%%%%%%%%
In this section we discuss the physical reasons behind the selective enrichment that gives rise to the trends such as in [C/O] presented in the previous section.
 
In a well mixed interstellar medium the gas is homogeneously enriched and has metal contribution from both the supernovae and the AGB stars. However in the early stages of the galaxy formation the properties of the galaxies were qualitatively different from what we see today for the normal galaxies. The hydrodynamical simulations of galaxy formation show that the newly formed galaxies have an abrupt history of star formation, that constitutes cycles of bursts leading to complete blow-out. 

During such a blow-out the galaxy becomes devoid of all its gas. Then the fresh pristine gas has to come in to form any new stars, however, the freshly arrived gas clouds will occupy the neighbourhoods of an older generation of stars already present in the galaxy from previous episodes of stars formation, and since this older population is capable of producing carbon if its age is $\gtrsim100$ Myr, that would lead to the formation of stars from the primordial gas enriched purely by the AGB.

\begin{figure}
\includegraphics[width=\linewidth]{fig_hist_element_mw_whyAGB_withvcmax_6.pdf}
\caption{The ratio of the metal mass acquired from AGB stars to that acquired from type  II SNe for star particles in {\sc eagle}  at redshift $z=6$ is plotted as a function of circular speed, $v_{\rm c,max}$ of the halo that contains the star particle. The ratio is normalized to the median value for the stars that live in haloes with $v_{\rm c,max}>100$ km~s$^{-1}$. The data points show the median value of the ratio and the error-bars (or the dark shaded region) represent the range of 40th to 60th percentile. The light shaded region depicts the range of 20th to 80th percentile. The scatter in the ratio increases with decreasing halo circular speed or halo mass, which implies that an increasingly large fraction of the stars in lower mass haloes are enriched either purely by AGB or type II SNe. Such a selective enrichment in low mass haloes is likely a consequence of the abrupt star formation history that involves cycles of rapid accretion and complete blow-out.}
\label{fig_vcmix}
\end{figure}

\begin{figure}
\includegraphics[width=\linewidth]{fig_hist_element_mw_whyAGB_vcmax_6.pdf}
\includegraphics[width=\linewidth]{fig_hist_element_mw_whyAGB_vcmax_8.pdf}
\includegraphics[width=\linewidth]{fig_hist_element_mw_whyAGB_vcmax_10.pdf}
\caption{The fraction of mass acquired from AGB is shown as a function of the fraction of mass acquired from the SNe type II for the metal poor stars at redshift, $z=6$ (top panel), 8 (middle panel) and 10 (bottom panel). The datapoints are colour-coded according to the maximum circular speed ($v_{\rm c, max}$) of the halo in which they live. Most of the star particles in the high mass galaxies (red points) are enriched via both channels indicating that the interstellar medium in such galaxies is well-mixed. Quite opposite for low mass galaxies, a significant number of stars are enriched either by the AGB channel or by the SNe type II, which reinstates the prevalence of poor mixing in such low mass galaxies. }
\label{fig_mix}
\end{figure}

This indeed is true for the galaxies in the {\sc eagle} simulation as seen in Fig.~\ref{fig_vcmix} and \ref{fig_mix} . Clearly there is a degeneracy in the enrichment of the star particles for low mass galaxies, since such galaxies have low escape speeds and are prone to strong outflows therefore going through a `breathing' phase featuring cycles of complete blow-out and fresh accretion. Thereafter fresh gas comes in that is then enriched by the well-aged AGB stars. 

\begin{figure}
\includegraphics[width=\linewidth]{fig_hist_element_mw_whyAGB_hist_2.pdf}
\caption{Upper panel : Number of star particles in a bin of halo mass at redshift 6. Distribution for the stars that are only enriched by AGB is shown as a blue histogra}
\end{figure}
